Measurement-Driven Adaptive Low-Overhead Implementation of Multi-Controlled Toffoli Gates

The Toffoli gate is a fundamental building block for quantum arithmetic and reversible logic, yet its efficient realization remains a major challenge in both near-term and fault-tolerant quantum architectures. Recent advances in dynamic quantum circuit capabilities, including mid-circuit measurement and classical feedforward, provide new opportunities for reducing the resource overhead of non-Clifford operations. In this work, we propose a set of dynamic decomposition strategies for multi-controlled Toffoli gates that exploit adaptive circuit execution and ancilla-assisted constructions. Our methods systematically reduce entangling-gate count, T-count, and T-depth compared with conventional static decompositions, while preserving fault-tolerance guarantees. Through analytical cost models and experimental evaluation, we demonstrate that relative-phase primitives and measurement-conditioned corrections enable scalable implementations with improved depth and resource efficiency.

==> figures/Table1.tex <==
%{\scriptsize
{ \setlength{\tabcolsep}{5pt}
%\begin{table*}[htbp]
\begin{sidewaystable}
  \caption{\small{Comparison of the dynamic Toffoli realizations based on \cite[Lemma 7.5]{PhysRevA.52.3457} and alternative decomposition structures with the corresponding clean ancilla based traditional implementations from \cite[Quantum Circuits 4.3]{Niel:2000}.}}
  \label{tab1}
%  \begin{minipage}{\textwidth}
%   \begin{center}
     \begin{tabular}{r||rrrr||rrr|rrr|rr||rrr|rrr|rr} \toprule 
   & \multicolumn{4}{c||}{\multirow{3}{*}{Clean Ancilla~\cite{Niel:2000}}} & \multicolumn{8}{c||}{ \cite[Lemma 7.5]{PhysRevA.52.3457} Based Dynamic Transformation} & \multicolumn{8}{c}{Alternate Dynamic Transformation}\\ \cmidrule(lr){6-13}\cmidrule(lr){14-21} %[1.9ex]\cmidrule{2-5}
%\textcolor{white}{\rule{0cm}{0.26cm}}
 %& clean ancilla  &  &  &  & Dynamic Barenco &  &  &  &  &  &  & Dynamic Proposed &  &  &  &  &  & 
\multirow{2}{*}{$n$}& \multicolumn{4}{c||}{} & \multicolumn{3}{c|}{ \multirow{2}{*}{$m=2$}} & \multicolumn{3}{c|}{ $m=2$,} & \multicolumn{2}{c||}{ Avg.} & \multicolumn{3}{c|}{ $m=2\textit{ if } n=3;$} & \multicolumn{3}{c|}{ $m=2$,} & \multicolumn{2}{c}{ Avg.}\\ %\cmidrule{2-5}\cmidrule{6-8} \cmidrule{9-11}\cmidrule{12-14}\cmidrule{15-17}\cmidrule{18-20}\cmidrule{21-23} %[1.9ex]
& \multicolumn{4}{c||}{} & \multicolumn{3}{c|}{ } & \multicolumn{3}{c|}{Unrolled} & \multicolumn{2}{c||}{  Improv.(\%)} & \multicolumn{3}{c|}{ $m = 3\textit{ othrwse. }$} & \multicolumn{3}{c|}{Unrolled} & \multicolumn{2}{c}{  Improv.(\%)}\\ \cmidrule(lr){2-5}
%\cmidrule(lr){6-13}\cmidrule(lr){14-21} %
\cmidrule(lr){6-8} \cmidrule(lr){9-11}\cmidrule(lr){12-13}\cmidrule(lr){14-16}\cmidrule(lr){17-19}\cmidrule(lr){20-21} %[1.9ex]
 & $m$ & $U$ & $CX$ & $D$ & $U$ & $CX$ & $D$ & $U$ & $CX$ & $D$ & $\delta_G$ & $\delta_{D}$ & $U$ & $CX$ & $D$ & $U$ & $CX$ & $D$ & $\delta_G$ & $\delta_{D}$  \\ \midrule
3 & 3 & 9 & 6 & 11 & 19 & 6 & 24 & 23 & 6 & 26 & -80.00 & -127.27 & 19 & 6 & 24 & 23 & 6 & 26 & -80.00 & -127.27 \\
4 & 5 & 21 & 12 & 28 & 33 & 10 & 39 & 39 & 10 & 42 & -39.39 & -44.65 & 40 & 14 & 46 & 46 & 12 & 48 & -69.70 & -67.86 \\
5 & 7 & 33 & 18 & 42 & 47 & 14 & 54 & 55 & 14 & 58 & -27.45 & -33.34 & 61 & 22 & 68 & 69 & 18 & 70 & -66.67 & -64.29 \\
6 & 9 & 45 & 24 & 56 & 61 & 18 & 69 & 71 & 18 & 74 & -21.74 & -27.68 & 82 & 30 & 90 & 92 & 24 & 92 & -65.22 & -62.50 \\
7 & 11 & 57 & 30 & 70 & 75 & 22 & 84 & 87 & 22 & 90 & -18.39 & -24.29 & 103 & 38 & 112 & 115 & 30 & 114 & -64.37 & -61.43 \\
8 & 13 & 69 & 36 & 84 & 89 & 26 & 99 & 103 & 26 & 106 & -16.19 & -22.03 & 124 & 46 & 134 & 138 & 36 & 136 & -63.81 & -60.71 \\
9 & 15 & 81 & 42 & 98 & 103 & 30 & 114 & 119 & 30 & 122 & -14.64 & -20.41 & 145 & 54 & 156 & 161 & 42 & 158 & -63.42 & -60.20 \\
10 & 17 & 93 & 48 & 112 & 117 & 34 & 129 & 135 & 34 & 138 & -13.48 & -19.20 & 166 & 62 & 178 & 184 & 48 & 180 & -63.12 & -59.82 \\
11 & 19 & 105 & 54 & 126 & 131 & 38 & 144 & 151 & 38 & 154 & -12.58 & -18.26 & 187 & 70 & 200 & 207 & 54 & 202 & -62.90 & -59.53 \\
12 & 21 & 117 & 60 & 140 & 145 & 42 & 159 & 167 & 42 & 170 & -11.87 & -17.50 & 208 & 78 & 222 & 230 & 60 & 224 & -62.71 & -59.29 \\
13 & 23 & 129 & 66 & 154 & 159 & 46 & 174 & 183 & 46 & 186 & -11.29 & -16.89 & 229 & 86 & 244 & 253 & 66 & 246 & -62.57 & -59.09 \\
14 & 25 & 141 & 72 & 168 & 173 & 50 & 189 & 199 & 50 & 202 & -10.80 & -16.37 & 250 & 94 & 266 & 276 & 72 & 268 & -62.44 & -58.93 \\
15 & 27 & 153 & 78 & 182 & 187 & 54 & 204 & 215 & 54 & 218 & -10.39 & -15.94 & 271 & 102 & 288 & 299 & 78 & 290 & -62.34 & -58.79 \\
16 & 29 & 165 & 84 & 196 & 201 & 58 & 219 & 231 & 58 & 234 & -10.04 & -15.56 & 292 & 110 & 310 & 322 & 84 & 312 & -62.25 & -58.67 \\\bottomrule
\multicolumn{21}{l}{$n\xrightarrow{}$MCT gate size; $m\xrightarrow{}$Number of qubits; $U\xrightarrow{}$Number of $1$-qubit gates; $\textit{CX}\xrightarrow{}$Number of $2$-qubit gates; $D\xrightarrow{}$Circuit depth;}\\
\multicolumn{21}{l}{$\delta_G$ / $\delta_D\xrightarrow{}$Average $\big((m=c_1), (m=c_2, \text{Unrolled})\big)$ increase in $(U+\textit{CX})$ / $D$ over traditional clean ancilla based realization.}\\\bottomrule
 %& & \multicolumn{2}{r}{Average}&\multicolumn{1}{r|}{33.15} & \multicolumn{2}{r}{Average}&\multicolumn{1}{r|}{23.20} & \multicolumn{2}{r}{Average}&\multicolumn{1}{r}{22.80} \\ \hline
      \end{tabular}
      
    %  \vspace{0.10in} $\#CNOT_d$ $\#CNOT_c$
    %&  \scriptsize{$\#CNOT_d$: CNOT gate count for dirty ancilla based decomposition, $\#CNOT_c$: CNOT gate count for dirty ancilla based decomposition}
      
      %\vspace{0.03in}
     % \scriptsize{$\#CNOT_c$: CNOT gate count for dirty ancilla based decomposition}
%    \end{center}
%     \end{minipage}
%\end{table*}
\end{sidewaystable}
}%}

==> figures/Table2.tex <==
%{\scriptsize
{ \setlength{\tabcolsep}{9pt}
\begin{table*}[htbp]
%\begin{sidewaystable}
  \caption{\small{Results for the dynamic realization of the Toffoli operation, comparing the method of \cite{PhysRevA.93.022311} with the proposed clean-ancilla–based dynamic decomposition.}}
  \label{tab2}
%  \begin{minipage}{\textwidth}
%   \begin{center}
     \begin{tabular}{rr||rrr||rrr||rrr} \toprule 
   & & \multicolumn{3}{c||}{Clean Ancilla~\cite{PhysRevA.93.022311}} & \multicolumn{3}{c||}{ Prop. Decomp.} & \multicolumn{3}{c}{Impr.(\%)}\\ \cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11} %[1.9ex]\cmidrule{2-5}
%\textcolor{white}{\rule{0cm}{0.26cm}}
 %& clean ancilla  &  &  &  & Dynamic Barenco &  &  &  &  &  &  & Dynamic Proposed &  &  &  &  &  & 
$n$& $a$ & $T_c$ & $T_d$ & $CX$ & $T_c$ & $T_d$ & $CX$ & $T_c$ & $T_d$ & $CX$ \\ \midrule
%\cmidrule(lr){6-13}\cmidrule(lr){14-21} %
%n     &    a     &  T-Count  & T-Depth   &  CNOT    & T-Count  & T-Depth  &   CNOT   &  T-Count    &  T-Depth    &    CNOT  \\
 4    &     1    &     15    &     11    &    12    &    11    &     7    &    10    &    26,67    &    36,36    &    16,67 \\
 5    &     2    &     23    &     19    &    18    &    15    &    11    &    14    &    34,78    &    42,11    &    22,22 \\
 6    &     3    &     31    &     27    &    24    &    19    &    15    &    18    &    38,71    &    44,44    &    25,00 \\
 7    &     4    &     39    &     35    &    30    &    23    &    19    &    22    &    41,03    &    45,71    &    26,67 \\
 8    &     5    &     47    &     43    &    36    &    27    &    23    &    26    &    42,55    &    46,51    &    27,78 \\
 9    &     6    &     55    &     51    &    42    &    31    &    27    &    30    &    43,64    &    47,06    &    28,57 \\
10    &     7    &     63    &     59    &    48    &    35    &    31    &    34    &    44,44    &    47,46    &    29,17 \\
11    &     8    &     71    &     67    &    54    &    39    &    35    &    38    &    45,07    &    47,76    &    29,63 \\
12    &     9    &     79    &     75    &    60    &    43    &    39    &    42    &    45,57    &    48,00    &    30,00 \\
13    &    10    &     87    &     83    &    66    &    47    &    43    &    46    &    45,98    &    48,19    &    30,30 \\
14    &    11    &     95    &     91    &    72    &    51    &    47    &    50    &    46,32    &    48,35    &    30,56 \\
15    &    12    &    103    &     99    &    78    &    55    &    51    &    54    &    46,60    &    48,48    &    30,77 \\
16    &    13    &    111    &    107    &    84    &    59    &    55    &    58    &    46,85    &    48,60    &    30,95 \\\bottomrule
\multicolumn{11}{l}{$n\xrightarrow{}$MCT gate size; $a\xrightarrow{}$Number of clean ancilla qubits; $T_c\xrightarrow{}$T-Count; $T_d \xrightarrow{}$T-Depth; } \\
\multicolumn{11}{l}{$CX \xrightarrow{}$CNOT-Count.}\\\bottomrule
 %& & \multicolumn{2}{r}{Average}&\multicolumn{1}{r|}{33.15} & \multicolumn{2}{r}{Average}&\multicolumn{1}{r|}{23.20} & \multicolumn{2}{r}{Average}&\multicolumn{1}{r}{22.80} \\ \hline
      \end{tabular}
      
    %  \vspace{0.10in} $\#CNOT_d$ $\#CNOT_c$
    %&  \scriptsize{$\#CNOT_d$: CNOT gate count for dirty ancilla based decomposition, $\#CNOT_c$: CNOT gate count for dirty ancilla based decomposition}
      
      %\vspace{0.03in}
     % \scriptsize{$\#CNOT_c$: CNOT gate count for dirty ancilla based decomposition}
%    \end{center}
%     \end{minipage}
\end{table*}
%\end{sidewaystable}
}%}


==> figures/c3_intermediate.tex <==
\scalebox{0.9}{
\Qcircuit @C=0.7em @R=0.24em @!R { \\
	 & \qw                 & \qw                 & \ctrl{3}            & \ctrl{1} & \qw                             & \ctrl{1} & \ctrl{1}  & \qw                             & \ctrl{1} & \qw\\
      & \qw                 & \ctrl{2}            & \qw                 & \targ    & \ctrl{2}                        & \targ    & \ctrl{1}  & \qw                             & \ctrl{1} & \qw\qw\\
 \lstick{\equiv\;\;\;\;\;}      & \ctrl{1}            & \qw                 & \qw                 & \qw      & \qw                             & \qw      & \targ     & \ctrl{1}                        & \targ     & \qw\\
      & \gate{\mathrm{U_2}} & \gate{\mathrm{U_3}} & \gate{\mathrm{U_3}} & \qw      & \gate{\mathrm{{U_3}\!^\dagger}} & \qw      & \qw       & \gate{\mathrm{{U_2}\!^\dagger}} & \qw       & \qw
\\ }}

==> figures/c3x.tex <==
\scalebox{0.92}{
\Qcircuit @C=0.7em @R=1.0em @!R { \\
	 	\lstick{{q}_{1} :  } & \ctrl{1} & \qw \\
	 	\lstick{{q}_{2} :  } & \ctrl{1} & \qw \\
	 	\lstick{{q}_{3} :  } & \ctrl{1} & \qw \\
	 	\lstick{{q}_{4} :  } & \targ    & \qw 
\\ }}

==> figures/cnx.tex <==
\scalebox{0.88}{
\Qcircuit @C=1.0em @R=1.15em @!R { \\
	 	\lstick{{q}_{1} :  }     & \ctrl{1} & \qw \\
	 	\lstick{{q}_{2} :  }     & \ctrl{2} & \qw \\
	 	\lstick{\cdots}          &          &     \\
	 	\lstick{{q}_{n-2} :  }   & \ctrl{1} & \qw \\
	 	\lstick{{q}_{n-1} :  }   & \ctrl{1} & \qw \\
	 	\lstick{{q}_{n} :  }     & \ctrl{1} & \qw \\
	 	\lstick{{q}_{n+1} :  }   & \targ    & \qw 
\\ }}

==> figures/cnx_dynamic.tex <==
\scalebox{0.9}{
\Qcircuit @C=0.9em @R=0.2em @!R { \\
\nghost{{q}_{1} :  }     &     \lstick{{q}_{1} :  }     &     \ctrl{1}     &     \meter     &         \push{{q}_{2} :\;\;}         &     \ctrl{1}     &     \gate{\mathrm{X}}     &     \ctrl{1}     &     \gate{\mathrm{X}}     &     \meter     &         \push{{q}_{3} :\;\;}         &     \ctrl{1}     &     \gate{\mathrm{X}}     &     \ctrl{1}     &     \gate{\mathrm{X}}     &     \meter\cwx[1]\\
\nghost{{q}_{4} :  }     &     \lstick{{q}_{4} :  }     &     \gate{\mathrm{U_{3}}}     &     \qw     &     \qw     &     \gate{\mathrm{U_{3}}}     &     \qw     &     \gate{\mathrm{{U_3}\!^\dagger}}     &     \qw     &     \qw     &     \qw     &     \gate{\mathrm{U_2}}     &     \qw     &     \gate{\mathrm{U_2\!^\dagger}}     &     \qw     &     \meter\\
\nghost{\mathrm{{c}_{1} :  }}     &     \lstick{\mathrm{{c}_{1} :  }}     &     \cw     &     \cw \ar @{<=} [-2,0]     &     \cw     &     \cw     &     \control \cw^(0.0){^{\mathtt{}}} \cwx[-2]     &     \cw     &     \control \cw^(0.0){^{\mathtt{}}} \cwx[-2]     &     \cw     &     \cw     &     \cw     &     \control \cw^(0.0){^{\mathtt{}}}     &     \cw     &     \control \cw^(0.0){^{\mathtt{}}}     &     \cw \\
\nghost{\mathrm{{c}_{2} :  }}     &     \lstick{\mathrm{{c}_{2} :  }}     &     \cw     &     \cw     &     \cw     &     \cw     &     \cw     &     \cw     &     \cw     &     \cw \ar @{<=} [-3,0]     &     \cw     &     \cw     &     \control \cw^(0.0){^{\mathtt{}}} \cwx[-3]     &     \cw     &     \control \cw^(0.0){^{\mathtt{}}} \cwx[-3]     &     \cw \\
\nghost{\mathrm{{c}_{3} :  }}     &     \lstick{\mathrm{{c}_{3} :  }}     &     \cw     &     \cw     &     \cw     &     \cw     &     \cw     &     \cw     &     \cw     &     \cw     &     \cw     &     \cw     &     \cw     &     \cw     &     \cw     &     \cw \ar @{<=} [-4,0]\\
\nghost{\mathrm{{c}_{4} :  }}     &     \lstick{\mathrm{{c}_{4} :  }}     &     \cw     &     \cw     &     \cw     &     \cw     &     \cw     &     \cw     &     \cw     &     \cw     &     \cw     &     \cw     &     \cw     &     \cw     &     \cw     &     \cw \ar @{<=} [-1,0]
\\ }}

==> figures/cnx_intermediate.tex <==
\scalebox{0.9}{
\Qcircuit @C=1.0em @R=0.2em @!R { \\
	 	& \qw                     & \ctrl{1}                  & \ctrl{1} & \qw                                 & \ctrl{1} & \ctrl{1}                              & \qw\\
	 	& \qw                     & \ctrl{2}                  & \ctrl{2} & \qw                                 & \ctrl{2} & \ctrl{2}                              & \qw\\
	 	& \push{\dots}            &                           &          & \push{\dots}                        &          &                                       &    \\
 \lstick{\equiv\;\;\;\;\;}      & \qw                     & \ctrl{1}                  & \ctrl{1} & \qw                                 & \ctrl{1} & \ctrl{1}                              & \qw\\
	 	& \qw                     & \ctrl{2}                  & \ctrl{1} & \qw                                 & \ctrl{1} & \ctrl{1}                              & \qw\\
	      & \ctrl{1}                & \qw                       & \targ    & \ctrl{1}                            & \targ    & \ctrlo{1}                             & \qw\\
	 	& \gate{\mathrm{V_{1,n}}} & \gate{\mathrm{V_{n-1,n}}} & \qw      & \gate{\mathrm{V_{1,n}\!^{\dagger}}} & \qw      & \gate{\mathrm{V_{n-2,n}\!^{\dagger}}} & \qw   \gategroup{2}{3}{8}{3}{.7em}{--}
\\}}

==> figures/dynamic_aimpb.tex <==
\scalebox{0.9}{
\Qcircuit @C=0.8em @R=0.5em @!R { 
\nghost{{q}_{0}} & \lstick{{q}_{0}} & \gate{\mathrm{X}} & \ctrl{1} & \ctrl{1} & \gate{\mathrm{X}} & \meter &  & \push{{q}_{1}\;} & \ctrl{1} & \ctrl{1} & \gate{\mathrm{X}} & \ctrl{1} & \gate{\mathrm{X}} & \meter \cwx[1] \\	
   \nghost{ {q}_{2} } & \lstick{ {q}_{2} } & \qw  & \targ & \gate{\mathrm{V}} & \qw & \qw & \qw & \qw & \targ & \gate{\mathrm{V}} & \qw & \gate{\mathrm{V^\dagger}} & \qw & \meter &  \\
	 	\nghost{\mathrm{{c_1} :  }} & \lstick{\mathrm{{c_0} :  }} & \cw & \cw & \cw & \cw & \dstick{_{_{\hspace{0.0em}}}} \cw \ar @{<=} [-2,0] & \cw & \cw & \cw & \cw  & \controlo \cw \cwx[-2] & \cw &  \controlo \cw \cwx[-2] & \cw \\
	 	\nghost{\mathrm{{c_2} :  }} & \lstick{\mathrm{{c_1} :  }} & \cw & \cw & \cw & \cw & \dstick{_{_{\hspace{0.0em}}}} \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \dstick{_{_{\hspace{0.0em}}}} \cw \ar @{<=} [-2,0]   \\   
	 	\nghost{\mathrm{{c_3} :  }} & \lstick{\mathrm{{c_2} :  }} & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw & \cw   & \dstick{_{_{\hspace{0.0em}}}} \cw \ar @{<=} [-1,0] 
\\}}

==> figures/trad_aimpb.tex <==
\scalebox{0.9}{
\Qcircuit @C=0.65em @R=0.5em @!R { 
	 	\lstick{{q}_{0}} & \qw  & \gate{X}  & \ctrl{2} & \ctrl{2} & \gate{X} & \qw & \gate{X}  & \ctrl{1}  & \qw &   \ctrl{1} & \gate{X} & \qw\\
            \lstick{{q}_{1}} & \ctrl{1} & \qw   & \qw & \qw & \qw & \ctrl{1} & \qw    & \targ & \ctrl{1} & \targ & \qw & \qw \\
            \lstick{{q}_{2}} & \targ  & \qw & \targ & \gate{\mathrm{V}} & \qw & \gate{\mathrm{V}} & \qw  & \qw & \gate{\mathrm{V^\dagger}} &  \qw    & \qw    & \qw
\\}}

==> sections/background_back.tex <==
\begin{figure}[t!]
    \centering
     \input{figures/trad_aimpb}
    \caption{An example 3-qubit quantum circuit consisting of NOT, CNOT, and controlled-$\sqrt{\text{NOT}}$ gates.}
    \label{trad-circuit}
\end{figure}
%A traditional quantum circuit is a cascade of unitary operations performed on a specific set of qubits before being measured~\cite{Niel:2000}.   
%Typically, unitary gates operating on $n$ qubits are represented by $2^n \times 2^n$ matrices. Typically a qubit can exists in basis states $|0 \rangle$ or $|1 \rangle$ or in superposition state, $\dirac{\psi} = \alpha |0 \rangle + \beta |1 \rangle$, where $\alpha$ and $\beta$ are complex coefficients and $|\alpha|^2 + |\beta|^2 = 1$. Measuring $\dirac{\psi}$ results in basis state of $|0 \rangle$ or $|1 \rangle$ with probabilities $|\alpha|^2$ and $|\beta|^2$ respectively, which is a non-unitary operation. 
%\cref{trad-circuit} shows the realization of a 3-qubit circuit using NOT ($X$), CNOT ($\textit{CX}$) and $CV$/$CV^\dagger$ gates where $V/V^\dagger$ indicates square-root of NOT operation, i.e. $X=(V)^2=(V^\dagger)^2$ and $VV^\dagger=I$. Here $q^D_0$ and $q^D_1$ are the control or data qubits and $q^A_0$ is a target or an answer qubit. 

A traditional quantum circuit is expressed as a sequence of unitary operations applied to a fixed set of qubits, followed by measurement~\cite{Niel:2000}. 
Unitary gates acting on $n$ qubits are represented by $2^{n} \times 2^{n}$ matrices. A single qubit can exist in one of the computational basis states $\ket{0}$ or $\ket{1}$, or in a superposition $\ket{\psi} = \alpha \ket{0} + \beta \ket{1}$, where $\alpha, \beta \in \mathbb{C}$ and $|\alpha|^{2} + |\beta|^{2} = 1$. Measuring $\ket{\psi}$ collapses it to $\ket{0}$ or $\ket{1}$ with probabilities $|\alpha|^{2}$ and $|\beta|^{2}$, respectively, which is a non-unitary process.
\Cref{trad-circuit} shows a 3-qubit circuit constructed using NOT ($X$), CNOT ($\mathit{CX}$), and controlled-$V$/$V^\dagger$ gates, where $V$ and $V^\dagger$ denote the square root of the NOT operation, i.e., $X = V^{2} = (V^\dagger)^{2}$ and $V V^\dagger = I$. 



%Certain non-unitaries~\cite{PhysRevLett.127.100501}, i.e. mid-circuit measurements, active-reset and classically controlled gates can be executed on real hardware thereby enabling a new class of dynamic quantum circuits.  
%An important feature of dynamic circuit is that it using deffered measurement principle~\cite{Niel:2000}
%enables intermediate measurement and releases qubits for resuse in further computation.
%Fig.~\ref{dyn-circuit} shows the dynamic realization of the 3-qubit cirucit (see Fig.~\ref{trad-circuit}) using two qubits. An iteration involves all the required operations between a two qubits before one of the qubit being measured.

Recent advances allow certain non-unitary operations, such as mid-circuit measurements, active reset, and classically conditioned gates, to be executed directly on hardware~\cite{PhysRevLett.127.100501}. These capabilities give rise to dynamic quantum circuits, which leverage the deferred measurement principle~\cite{Niel:2000} to incorporate intermediate measurements and subsequently recycle qubits for later stages of the computation.
\Cref{dyn-circuit} illustrates the dynamic realization of the 3-qubit circuit depicted in \Cref{trad-circuit}, implemented using only two qubits. Each iteration performs the required operations on the two available qubits before one of them is measured and reused.

\begin{figure}[htbp!]
    \centering
     \input{figures/dynamic_aimpb}
    \caption{Dynamic 2-qubit realization of the 3-qubit circuit using qubit recycling.}
    \label{dyn-circuit}
\end{figure}



==> sections/qubit-recycling.tex <==
%Ceartain decomposition structure for Toffoli gates are not suitable for dynamic transforamtion recycling qubits. In~\cite{10546695,10137250}, the qubit reordering problem is specifically addressed by using controlled unitaries of the form $C\sqrt[n]{X}/C\sqrt[n]{X}^\dagger$ for implementation. A $n$-qubit 
%MCT operation when controlled unitaries of the form $CU_{k}$ where $U_{k}=\sqrt[\leftroot{1}\uproot{-1}2^{k}]{I}$, $k\in \mathbb{Z^+}$ are realizable~\cite[Lemma 7.5]{PhysRevA.52.3457}. Considering $U_k = \sqrt[\leftroot{1}\uproot{-1}2^{k-1}]{Z}$, a $CU_{k}/C{U_k}\!^\dagger$ operation can be realized as a $CP_{k}/C{P_k}\!^\dagger$ operation using $CX$ and single-qubit $\pm\frac{\pi}{2^k}$ phase operation. Assuming $U_k = \sqrt[\leftroot{1}\uproot{-1}2^{k-1}]{X}$, then $CU_{k}/C{U_k}\!^\dagger$ operation is derived by introducing a pair of $H$ operations (i.e., $X^r = HZ^rH$ for all $r\in\mathbb{R}$). %in the realization.  

%Fig.~\ref{fig:c3x_ancillafree} shows an intermediate level representation of a $4$-qubit MCT operation using controlled-$U_2$ and -$U_3$ gates where $U_k = \sqrt[\leftroot{1}\uproot{-1}2^{k-1}]{X}$.
%The realization allows reordering of qubits thereby enabling qubit recycling as shown in Fig.~\ref{fig:cnx_dynamic1_rolled}.



%Instead of considering these $2^k$-th root of identity operations, another structure considered in~\cite{10546695} employing controlled unitaries 
%of the form $CV_{k,n}$, $k\in \mathbb{Z^+}$ for $1\leqslant k\leqslant n-2$ where $V_{k,n}=\sqrt[\leftroot{5}\uproot{2}\frac{2n}{k}]{I}$ for the dynamic transformation of Toffoli operation.
%Fig.~\ref{fig:cnx_ancillafree} shows the realization of a $(n+1)$-qubit Toffoli operation using $\textit{CX}$ and $CV_{k,n}$ gates. This compared to previous approach requires larger controlled-phase gates, i.e. $\sqrt[\leftroot{5}\uproot{2}\frac{2n}{k}]{I} > \sqrt[\leftroot{1}\uproot{-1}2^{k-1}]{X}$, leading to more economical fault-tolerant realization~\cite{10.5555/2685188.2685198}. 


Certain decomposition structures for Toffoli gates are not suitable for dynamic transformations that rely on qubit recycling. 
In~\cite{10546695,10137250}, the qubit reordering problem is specifically addressed using controlled unitaries of the form 
$C\sqrt[n]{X}$/$C\sqrt[n]{X}^\dagger$. An $n$-qubit Toffoli operation can be realized when controlled unitaries of the form $CU_{k}$, where $U_{k} = \sqrt[\leftroot{1}\uproot{-1}2^{k}]{I}$ and $k \in \mathbb{Z}^{+}$, are available~\cite[Lemma~7.5]{PhysRevA.52.3457}. 
Considering $U_{k} = \sqrt[\leftroot{1}\uproot{-1}2^{k-1}]{Z}$, a $CU_{k}$/$CU_{k}^{\dagger}$ operation can be implemented as a $CP_{k}$/$CP_{k}^{\dagger}$ operation using $\mathit{CX}$ and single-qubit $\pm\!\frac{\pi}{2^{k}}$ phase rotations.  
Alternatively, if $U_{k} = \sqrt[\leftroot{1}\uproot{-1}2^{k-1}]{X}$, then $CU_{k}$/$CU_{k}^{\dagger}$ can be obtained by 
introducing a pair of Hadamard gates, using the identity $X^{r} = H Z^{r} H$ for all $r \in \mathbb{R}$.

\begin{figure}[htbp!]
    \centering
     \begin{subfigure}[b]{0.08\textwidth}
         \centering
         \input{figures/c3x}
         \vspace{0.15cm}
         \caption{}
         \label{fig:c3x}
     \end{subfigure}\quad\quad\quad
     %\hspace{-0.4cm}
     \begin{subfigure}[b]{0.25\textwidth}
         \centering
         \input{figures/c3_intermediate}
         \caption{}
         \label{fig:c3x_intermediate}
     \end{subfigure}
    \caption{
    Toffoli realization for qubit recycling. 
(a) A 4-qubit Toffoli gate. 
(b) Its Decomposition using controlled-$X$, controlled-$U_{2}$/$U_{2}^{\dagger}$, and controlled-$U_{3}$/$U_{3}^{\dagger}$ gates~\cite[Lemma~7.5]{PhysRevA.52.3457}.
    %Ancilla free realization: (a) A $4$-qubit MCT gate.  
    %(b) An ancilla free decomposed MCT operation using controlled-$X$, -$U_2/{U_2}\!^\dagger$ and -$U_3/{U_3}\!^\dagger$ gates~\cite[Lemma~7.5]{PhysRevA.52.3457}.
    }\label{fig:c3x_ancillafree}
\end{figure}

\Cref{fig:c3x_ancillafree} illustrates an intermediate-level decomposition of a 4-qubit MCT gate using controlled-$U_{2}$ 
and controlled-$U_{3}$ operations with $U_{k} = \sqrt[\leftroot{1}\uproot{-1}2^{k-1}]{X}$. 
This structure supports qubit reordering, thereby enabling qubit recycling as demonstrated in 
\Cref{fig:cnx_dynamic}.

\begin{figure*}[t!]
    \centering
    
         \input{figures/cnx_dynamic}
        % \vspace{-0.03cm}
    
    \caption{Dynamic 2-qubit realization of a 4-qubit Toffoli operation using controlled-$U_{2}$ and controlled-$U_{3}$ gates, classically controlled-$X$ operations, and three iterations, where $U_{k} = \sqrt[\leftroot{1}\uproot{-1}2^{k-1}]{X}$. %and $U_k{U_k}\!^\dagger = I$.
    }
    \label{fig:cnx_dynamic}
\end{figure*}


Instead of using $2^{k}$-th roots of the identity, an alternative structure considered in~\cite{10546695} employs controlled 
unitaries of the form $CV_{k,n}$, for $1 \leqslant k \leqslant n-2$, where 
$
V_{k,n} = \sqrt[\leftroot{5}\uproot{2}\frac{2n}{k}]{I},
$
to achieve dynamic transformations of Toffoli operations. 
\Cref{fig:cnx_ancillafree} shows a realization of an $(n+1)$-qubit Toffoli gate using $\mathit{CX}$ and $CV_{k,n}$ 
operations. Compared to the previous approach, this method requires larger controlled-phase gates (i.e., 
$\sqrt[\leftroot{5}\uproot{2}\frac{2n}{k}]{I} > \sqrt[\leftroot{1}\uproot{-1}2^{k-1}]{X}$), which leads to a more 
resource-efficient fault-tolerant implementation~\cite{10.5555/2685188.2685198}.





\begin{figure*}[htbp!]
    \centering
     \begin{subfigure}[b]{0.02\textwidth}
         \centering
         \input{figures/cnx}
         \vspace{0.17cm}
         \caption{}
         \label{fig:cnx}
     \end{subfigure}\qquad\quad%\quad
     \hspace{0.8cm}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \input{figures/cnx_intermediate}
         \caption{}
         \label{fig:cnx_proposed}
     \end{subfigure}
    \caption{Decomposition of an $(n+1)$-qubit Toffoli gate using $\mathit{CX}$ and $CV_{k,n}$ operations for $1 \leqslant k \leqslant n-2$, where $V_{k,n} = \sqrt[\leftroot{5}\uproot{2}\frac{n}{k}]{X}$. 
(a) The $(n+1)$-qubit Toffoli gate. 
(b) Its  decomposition using $\mathit{CX}$ and $CV_{k,n}$ gates.}\label{fig:cnx_ancillafree}
\end{figure*}
